Language Models Can Teach Themselves to Program Better

Recent Language Models (LMs) achieve breakthrough performance in code generation when trained on human-authored problems, even solving some competitive-programming problems. Self-play has proven useful in games such as Go, and thus it is natural to ask whether LMs can generate their own instructive programming problems to improve their performance. We show that it is possible for an LM to synthesize programming problems and solutions, which are filtered for correctness by a Python interpreter. The LM's performance is then seen to improve when it is fine-tuned on its own synthetic problems and verified solutions; thus the model 'improves itself' using the Python interpreter. Problems are specified formally as programming puzzles [Schuster et al., 2021], a code-based problem format where solutions can easily be verified for correctness by execution. In experiments on publicly-available LMs, test accuracy more than doubles. This work demonstrates the potential for code LMs, with an interpreter, to generate instructive problems and improve their own performance.

==> scraps/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> scraps/train_155.tex <==
\begin{pylittledisplay}

# Training problem 1
def f(s: str):
    return s.count('o') == 1000 and s.count('oo') == 0

# Training problem 2
def f(li: List[int]):
    return sorted(li) == list(range(999)) and all(li[i] != i for i in range(len(li)))

# Training problem 3
def f(li: List[int]):
    return all([li.count(i) == i for i in range(10)])

# Training problem 4
def f(s: str):
    return str(8 ** 2888).count(s) > 8 and len(s) == 3

# Training problem 5
def f(li: List[int]):
    return ["The quick brown fox jumps over the lazy dog"[i] for i in li] == list(
        "The five boxing wizards jump quickly")

# Training problem 6
def f(ls: List[str]):
    return min(ls) == max(ls) == str(len(ls))

# Training problem 7
def f(x: float):
    return str(x - 3.1415).startswith("123.456")

# Training problem 8
def f(li: List[int]):
    return all(sum(li[:i]) == 2 ** i - 1 for i in range(20))

# Training problem 9
def f(i: int):
    return len(str(i + 1000)) > len(str(i + 1001))

# Training problem 10
def f(li: List[int]):
    return {i + j for i in li for j in li} == {0, 1, 2, 3, 4, 5, 6, 17, 18, 19, 20, 34}

# Training problem 11
def f(li: List[int]):
    return all([li[i] != li[i + 1] for i in range(10)]) and len(set(li)) == 3

# Training problem 12
def f(ls: List[str]):
    return tuple(ls) in zip('dee', 'doo', 'dah!')

# Training problem 13
def f(s: str):
    return sorted(s) == sorted('Permute me true') and s == s[::-1]

# Training problem 14
def f(li: List[int]):
    return li[li[0]] != li[li[1]] and li[li[li[0]]] == li[li[li[1]]]

# Training problem 15
def f(l: List[int]):
    return all(i in range(1000) and abs(i * i - j * j) >= 10 for i in l for j in l if i != j) and len(set(l)) > 995

# Training problem 16
def f(hands: List[int], target_angle=45):
    h, m = hands
    assert 0 < h <= 12 and 0 <= m < 60
    hour_angle = 30 * h + m / 2
    minute_angle = 6 * m
    return abs(hour_angle - minute_angle) in [target_angle, 360 - target_angle]

# Training problem 17
def f(daygroups: List[List[List[int]]]):
    assert len(daygroups) == 7
    assert all(len(groups) == 5 and {i for g in groups for i in g} == set(range(15)) for groups in daygroups)
    assert all(len(g) == 3 for groups in daygroups for g in groups)
    return len({(i, j) for groups in daygroups for g in groups for i in g for j in g}) == 15 * 15

# Training problem 18
def f(n: int):
    for i in range(5):
        assert n % 5 == 1
        n -= 1 + (n - 1) // 5
    return n > 0 and n % 5 == 1

# Training problem 19
def f(coords: List[List[int]], side=10, num_points=20):
    for i1 in range(len(coords)):
        x1, y1 = coords[i1]
        assert 0 <= x1 < side and 0 <= y1 < side
        for i2 in range(i1):
            x2, y2 = coords[i2]
            for i3 in range(i2):
                x3, y3 = coords[i3]
                assert x1 * (y2 - y3) + x2 * (y3 - y1) + x3 * (y1 - y2) != 0
    return len({(a, b) for a, b in coords}) == len(coords) >= num_points

# Training problem 20
def f(stamps: List[int], target=80, max_stamps=4, options=[10, 32, 8]):
    for s in stamps:
        assert s in options
    return len(stamps) <= max_stamps and sum(stamps) == target

# Training problem 21
def f(xy_sides: List[List[int]]):
    n = max(x + side for x, y, side in xy_sides)
    assert len({side for x, y, side in xy_sides}) == len(xy_sides) > 1
    for x, y, s in xy_sides:
        assert 0 <= y < y + s <= n and 0 <= x
        for x2, y2, s2 in xy_sides:
            assert s2 <= s or x2 >= x + s or x2 + s2 <= x or y2 >= y + s or y2 + s2 <= y

    return sum(side ** 2 for x, y, side in xy_sides) == n ** 2

# Training problem 22
def f(n: int, lace="bbrbrbbbbbbrrrrrrrbrrrrbbbrbrrbbbrbrrrbrrbrrbrbbrrrrrbrbbbrrrbbbrbbrbbbrbrbb"):
    sub = lace[n: n + len(lace) // 2]
    return n >= 0 and lace.count("r") == 2 * sub.count("r") and lace.count("b") == 2 * sub.count("b")

# Training problem 23
def f(n: int):
    s = str(n * n)
    for i in "0123456789":
        assert s.count(i) == 1
    return True

# Training problem 24
def f(s: str):
    return set(s) <= set("18-+*/") and s.count("8") == 2 and s.count("1") == 1 and eval(s) == 63

# Training problem 25
def f(s: str):
    return set(s) <= set("18-+*/") and s.count("8") == 3 and s.count("1") == 1 and eval(s) == 63

# Training problem 26
def f(moves: List[List[int]], capacities=[8, 5, 3], init=[8, 0, 0], goal=[4, 4, 0]):
    state = init.copy()

    for [i, j] in moves:
        assert min(i, j) >= 0, "Indices must be non-negative"
        assert i != j, "Cannot pour from same state to itself"
        n = min(capacities[j], state[i] + state[j])
        state[i], state[j] = state[i] + state[j] - n, n

    return state == goal

# Training problem 27
def f(li: List[int], words=['SEND', 'MORE', 'MONEY']):
    assert len(li) == len(words) and all(i > 0 and len(str(i)) == len(w) for i, w in zip(li, words))
    assert len({c for w in words for c in w}) == len({(d, c) for i, w in zip(li, words) for d, c in zip(str(i), w)})
    return sum(li[:-1]) == li[-1]

# Training problem 28
def f(s: str, word="antidisestablishmentarianism", max_len=10):
    if len(word) <= max_len:
        return word == s
    return int(s[1:-1]) == len(word[1:-1]) and word[0] == s[0] and word[-1] == s[-1]

# Training problem 29
def f(corners: List[List[int]], m=10, n=9, a=5, target=4):
    covered = {(i + x, j + y) for i, j in corners for x in range(a) for y in range(a)}
    assert len(covered) == len(corners) * a * a, "Double coverage"
    return len(corners) <= target and covered.issuperset({(x, y) for x in range(m) for y in range(n)})

# Training problem 30
def f(lb: List[bool], trips=[[1, 1, 0], [1, 0, 0], [0, 0, 0], [0, 1, 1], [0, 1, 1], [1, 1, 1], [1, 0, 1]]):
    return len(lb) == len(trips) and all(
        (b is True) if sum(s) >= 2 else (b is False) for b, s in zip(lb, trips))

# Training problem 31
def f(n: int, scores=[100, 95, 80, 70, 65, 9, 9, 9, 4, 2, 1], k=6):
    assert all(scores[i] >= scores[i + 1] for i in range(len(scores) - 1)), "Hint: scores are non-decreasing"
    return all(s >= scores[k] and s > 0 for s in scores[:n]) and all(s < scores[k] or s <= 0 for s in scores[n:])

# Training problem 32
def f(t: str, s="Problems"):
    i = 0
    for c in s.lower():
        if c in "aeiouy":
            continue
        assert t[i] == ".", f"expecting `.` at position {i}"
        i += 1
        assert t[i] == c, f"expecting `{c}`"
        i += 1
    return i == len(t)

# Training problem 33
def f(squares: List[List[int]], m=10, n=5, target=50):
    covered = []
    for i1, j1, i2, j2 in squares:
        assert (0 <= i1 <= i2 < m) and (0 <= j1 <= j2 < n) and (j2 - j1 + i2 - i1 == 1)
        covered += [(i1, j1), (i2, j2)]
    return len(set(covered)) == len(covered) == target

# Training problem 34
def f(n: int, ops=['x++', '--x', '--x'], target=19143212):
    for op in ops:
        if op in ["++x", "x++"]:
            n += 1
        else:
            assert op in ["--x", "x--"]
            n -= 1
    return n == target

# Training problem 35
def f(n: int, s="aaAab", t="aAaaB"):
    if n == 0:
        return s.lower() == t.lower()
    if n == 1:
        return s.lower() > t.lower()
    if n == -1:
        return s.lower() < t.lower()
    return False

# Training problem 36
def f(s: str, word="konjac"):
    for i in range(len(word)):
        if i == 0:
            if s[i] != word[i].upper():
                return False
        else:
            if s[i] != word[i]:
                return False
    return True

# Training problem 37
def f(t: str, s="abbbcabbac", target=7):
    i = 0
    for c in t:
        while c != s[i]:
            i += 1
        i += 1
    return len(t) >= target and all(t[i] != t[i + 1] for i in range(len(t) - 1))

# Training problem 38
def f(delta: List[int], nums=[[1, 2, 3], [9, -2, 8], [17, 2, 50]]):
    return all(sum(vec[i] for vec in nums) + delta[i] == 0 for i in range(3))

# Training problem 39
def f(n: int, a=17, b=100, c=20):
    return n + a == sum([b * i for i in range(c)])

# Training problem 40
def f(n: int, v=17, w=100):
    for i in range(n):
        assert v <= w
        v *= 3
        w *= 2
    return v > w

# Training problem 41
def f(res: int, m=1234578987654321, n=4):
    for i in range(n):
        m = (m - 1 if m % 10 else m // 10)
    return res == m

# Training problem 42
def f(n: int, pairs=[[3, 0], [17, 1], [9254359, 19], [123, 9254359], [0, 123]]):
    assert sum(p - m for p, m in pairs) == 0, "oo"
    tot = 0
    success = False
    for p, m in pairs:
        tot -= m
        tot += p
        assert tot <= n
        if tot == n:
            success = True
    return success

# Training problem 43
def f(s_case: str, s="CanYouTellIfItHASmoreCAPITALS"):
    caps = 0
    for c in s:
        if c != c.lower():
            caps += 1
    return s_case == (s.upper() if caps > len(s) // 2 else s.lower())

# Training problem 44
def f(inds: List[int], string="enlightenment"):
    return inds == sorted(inds) and "".join(string[i] for i in inds) == "intelligent"

# Training problem 45
def f(d: int, n=123456789):
    return d > n and all(i in "47" for i in str(str(d).count("4") + str(d).count("7")))

# Training problem 46
def f(s: str, target="reverse me", reverse=True):
    return (s[::-1] == target) == reverse

# Training problem 47
def f(s: str, a=5129, d=17):
    return s.count("a") == a and s.count("d") == d and len(s) == a + d

# Training problem 48
def f(nums: List[int], a=100, b=1000, count=648):
    assert all(len(str(n)) == len(set(str(n))) and a <= n <= b for n in nums)
    return len(set(nums)) >= count

# Training problem 49
def f(tot: int, nums=[2, 8, 25, 18, 99, 11, 17, 16], thresh=17):
    return tot == sum(1 if i < thresh else 2 for i in nums)

# Training problem 50
def f(s: str, chars=['o', 'h', 'e', 'l', ' ', 'w', '!', 'r', 'd']):
    for c in chars:
        if c not in s:
            return False
    return True

# Training problem 51
def f(ans: List[List[int]], target=17):
    for i in range(len(ans)):
        a, b = ans[i]
        if b - a >= 2:
            target -= 1
    return target == 0

# Training problem 52
def f(indexes: List[int], target=[1, 3, 4, 2, 5, 6, 7, 13, 12, 11, 9, 10, 8]):
    for i in range(1, len(target) + 1):
        if target[indexes[i - 1] - 1] != i:
            return False
    return True

# Training problem 53
def f(s: str, n=7012):
    return int(str(5 ** n)[:-2] + s) == 5 ** n

# Training problem 54
def f(states: List[str], start="424", combo="778", target_len=12):
    assert all(len(s) == len(start) for s in states) and all(c in "0123456789" for s in states for c in s)
    for a, b in zip([start] + states, states + [combo]):
        assert sum(i != j for i, j in zip(a, b)) == 1
        assert all(abs(int(i) - int(j)) in {0, 1, 9} for i, j in zip(a, b))

    return len(states) <= target_len

# Training problem 55
def f(states: List[str], start="424", combo="778", target_len=12):
    return all(sum((int(a[i]) - int(b[i])) ** 2 % 10 for i in range(len(start))) == 1
               for a, b in zip([start] + states, states[:target_len] + [combo]))

# Training problem 56
def f(s: str, perm="qwertyuiopasdfghjklzxcvbnm", target="hello are you there?"):
    return "".join((perm[(perm.index(c) + 1) % len(perm)] if c in perm else c) for c in s) == target

# Training problem 57
def f(lists: List[List[int]], items=[5, 4, 9, 4, 5, 5, 5, 1, 5, 5], length=4):
    a, b = lists
    assert len(a) == len(b) == length
    assert len(set(a)) == len(a)
    assert len(set(b)) == 1
    for i in a + b:
        assert (a + b).count(i) <= items.count(i)
    return True

# Training problem 58
def f(seq: List[int], n=10000, length=5017):
    return all(i in [1, 2] for i in seq) and sum(seq) == n and len(seq) == length

# Training problem 59
def f(start: int, k=3, upper=6, seq=[17, 1, 2, 65, 18, 91, -30, 100, 3, 1, 2]):
    return 0 <= start <= len(seq) - k and sum(seq[start:start + k]) <= upper

# Training problem 60
def f(start: int, k=3, lower=150, seq=[3, 1, 2, 65, 18, 91, -30, 100, 0, 19, 52]):
    return 0 <= start <= len(seq) - k and sum(seq[start:start + k]) >= lower

# Training problem 61
def f(start: int, k=3, lower=100000, seq=[91, 1, 2, 64, 18, 91, -30, 100, 3, 65, 18]):
    prod = 1
    for i in range(start, start + k):
        prod *= seq[i]
    return prod >= lower

# Training problem 62
def f(nums: List[int], tot=12345, n=5):
    return len(nums) == len(set(nums)) == n and sum(nums) == tot and all(i >= i % 2 > 0 for i in nums)

# Training problem 63
def f(rotations: List[int], target="wonderful", upper=69):
    s = "abcdefghijklmnopqrstuvwxyz"
    assert len(rotations) == len(target)
    for r, c in zip(rotations, target):
        s = s[r:] + s[:r]
        assert s[0] == c

    return sum(abs(r) for r in rotations) <= upper

# Training problem 64
def f(bills: List[int], denominations=[1, 25, 35, 84], n=980, max_len=14):
    return sum(bills) == n and all(b in denominations for b in bills) and len(bills) <= max_len

# Training problem 65
def f(sides: List[int], options=[2, 512, 1024], n=340282366920938463463374607431768211456, max_dim=13):
    prod = 1
    for b in sides:
        prod *= b
    return prod == n and set(sides) <= set(options) and len(sides) <= max_dim

# Training problem 66
def f(x: float, coeffs=[2.5, 1.3, -0.5]):
    a, b, c = coeffs
    return abs(a * x ** 2 + b * x + c) < 1e-6

# Training problem 67
def f(roots: List[float], coeffs=[1.3, -0.5]):
    b, c = coeffs
    r1, r2 = roots
    return abs(r1 + r2 + b) + abs(r1 * r2 - c) < 1e-6

# Training problem 68
def f(x: str, s=679):
    return s == sum([int(d) for d in x])

# Training problem 69
def f(z: float, v=9, d=0.0001):
    return int(z * 1 / d % 10) == v

# Training problem 70
def f(x: List[int], a=7, s=5, e=200):
    return x[0] == a and x[-1] <= e and (x[-1] + s > e) and all([x[i] + s == x[i + 1] for i in range(len(x) - 1)])

# Training problem 71
def f(e: List[int], a=2, b=-1, c=1, d=2021):
    x = e[0] / e[1]
    return abs(a * x + b - c * x - d) < 10 ** -5

# Training problem 72
def f(x: int, a=253532, b=1230200):
    if x > 0 or a > 50:
        return x - a == b
    else:
        return x + a == b

# Training problem 73
def f(x: int, a=4, b=54368639):
    if a == 1:
        return x % 2 == 0
    elif a == -1:
        return x % 2 == 1
    else:
        return x + a == b

# Training problem 74
def f(x: List[int], n=5, s=19):
    return len(x) == n and sum(x) == s and all([a > 0 for a in x])

# Training problem 75
def f(x: List[int], n=4, s=2021):
    return len(x) == n and sum(x) == s and len(set(x)) == n

# Training problem 76
def f(x: str, s=['a', 'b', 'c', 'd', 'e', 'f'], n=4):
    return len(x) == n and all([x[i] == s[i] for i in range(n)])

# Training problem 77
def f(x: List[int], t=677, a=43, e=125, s=10):
    non_zero = [z for z in x if z != 0]
    return t == sum([x[i] for i in range(a, e, s)]) and len(set(non_zero)) == len(non_zero) and all(
        [x[i] != 0 for i in range(a, e, s)])

# Training problem 78
def f(x: List[int], t=50, n=10):
    assert all([v > 0 for v in x])
    s = 0
    i = 0
    for v in sorted(x):
        s += v
        if s > t:
            return i == n
        i += 1
    return i == n

# Training problem 79
def f(s: str, s1="a", s2="b", count1=50, count2=30):
    return s.count(s1) == count1 and s.count(s2) == count2 and s[:10] == s[-10:]

# Training problem 80
def f(s: str, substrings=['foo', 'bar', 'baz', 'oddball']):
    return all(sub in s[i::len(substrings)] for i, sub in enumerate(substrings))

# Training problem 81
def f(s: str, substrings=['foo', 'bar', 'baz']):
    return all(sub in s and sub[::-1] in s for sub in substrings)

# Training problem 82
def f(s: str, strings=['cat', 'dog', 'bird', 'fly', 'moose']):
    return s in strings and sum(t > s for t in strings) == 1

# Training problem 83
def f(s: str, strings=['cat', 'dog', 'bird', 'fly', 'moose']):
    return s[::-1] in strings and sum(t < s[::-1] for t in strings) == 1

# Training problem 84
def f(s: str, target="foobarbazwow", length=6):
    return target[(len(target) - length) // 2:(len(target) + length) // 2] == s

# Training problem 85
def f(substring: str, string="moooboooofasd", count=2):
    return string.count(substring) == count

# Training problem 86
def f(t: str, s="))(Add)some))parens()to()(balance(()(()(me!)(((("):
    for i in range(len(t) + 1):
        depth = t[:i].count("(") - t[:i].count(")")
        assert depth >= 0
    return depth == 0 and s in t

# Training problem 87
def f(squares: List[List[int]], m=8, n=8):
    k = min(m, n)
    assert all(i in range(m) and j in range(n) for i, j in squares) and len(squares) == k
    return 4 * k == len({t for i, j in squares for t in [('row', i), ('col', j), ('SE', i + j), ('NE', i - j)]})

# Training problem 88
def f(tour: List[List[int]], m=8, n=8):
    assert all({abs(i1 - i2), abs(j1 - j2)} == {1, 2} for [i1, j1], [i2, j2] in zip(tour, tour[1:])), 'legal moves'
    return sorted(tour) == [[i, j] for i in range(m) for j in range(n)]  # cover every square once

# Training problem 89
def f(path: List[List[int]], m=8, n=8, target=35):
    def legal_move(m):
        (a, b), (i, j) = m
        return {abs(i - a), abs(j - b)} == {1, 2}

    def legal_quad(m1, m2):  # non-overlapping test: parallel or bounding box has (width - 1) * (height - 1) >= 5
        (i1, j1), (i2, j2) = m1
        (a1, b1), (a2, b2) = m2
        return (len({(i1, j1), (i2, j2), (a1, b1), (a2, b2)}) < 4  # adjacent edges in path, ignore
                or (i1 - i2) * (b1 - b2) == (j1 - j2) * (a1 - a2)  # parallel
                or (max(a1, a2, i1, i2) - min(a1, a2, i1, i2)) * (max(b1, b2, j1, j2) - min(b1, b2, j1, j2)) >= 5
                # far
                )

    assert all(i in range(m) and j in range(n) for i, j in path), "move off board"
    assert len({(i, j) for i, j in path}) == len(path), "visited same square twice"

    moves = list(zip(path, path[1:]))
    assert all(legal_move(m) for m in moves), "illegal move"
    assert all(legal_quad(m1, m2) for m1 in moves for m2 in moves), "intersecting move pair"

    return len(path) >= target

# Training problem 90
def f(path: List[List[int]], m=10, n=10, target=62):
    def legal_move(m):
        (a, b), (i, j) = m
        return {abs(i - a), abs(j - b)} == {1, 2}

    def legal_quad(m1, m2):  # non-overlapping test: parallel or bounding box has (width - 1) * (height - 1) >= 5
        (i1, j1), (i2, j2) = m1
        (a1, b1), (a2, b2) = m2
        return (len({(i1, j1), (i2, j2), (a1, b1), (a2, b2)}) < 4  # adjacent edges in path, ignore
                or (i1 - i2) * (b1 - b2) == (j1 - j2) * (a1 - a2)  # parallel
                or (max(a1, a2, i1, i2) - min(a1, a2, i1, i2)) * (max(b1, b2, j1, j2) - min(b1, b2, j1, j2)) >= 5
                # far
                )

    assert all(i in range(m) and j in range(n) for i, j in path), "move off board"
    assert len({(i, j) for i, j in path}) == len(path), "visited same square twice"

    moves = list(zip(path, path[1:]))
    assert all(legal_move(m) for m in moves), "illegal move"
    assert all(legal_quad(m1, m2) for m1 in moves for m2 in moves), "intersecting move pair"

    return len(path) >= target

# Training problem 91
def f(position: List[List[int]], target=[[1, 3], [1, 4], [2, 5]]):
    live = {x + y * 1j for x, y in position}  # complex numbers encode live cells
    deltas = (1j, -1j, 1, -1, 1 + 1j, 1 - 1j, -1 + 1j, -1 - 1j)
    visible = {z + d for z in live for d in deltas}
    next_step = {z for z in visible if sum(z + d in live for d in deltas) in ([2, 3] if z in live else [3])}
    return next_step == {x + y * 1j for x, y in target}

# Training problem 92
def f(init: List[List[int]], period=4):
    live = {x + y * 1j for x, y in init}  # use complex numbers
    init_tot = sum(live)
    target = {z * len(live) - init_tot for z in live}
    deltas = (1j, -1j, 1, -1, 1 + 1j, 1 - 1j, -1 + 1j, -1 - 1j)

    for t in range(period):
        visible = {z + d for z in live for d in deltas}
        live = {z for z in visible if 3 - (z in live) <= sum(z + d in live for d in deltas) <= 3}
        tot = sum(live)
        if {z * len(live) - tot for z in live} == target:
            return t + 1 == period and tot != init_tot

# Training problem 93
def f(moves: List[List[int]], initial_state=[5, 9, 3, 11, 18, 25, 1, 2, 4, 1]):

    def bot_move():  # bot takes objects from the largest heap to make it match the second largest heap
        vals = sorted(state, reverse=True)
        i_largest = state.index(vals[0])  # largest heap
        state[i_largest] -= max(vals[0] - vals[1], 1)  # must take some, take 1 in case of tie

    state = initial_state[:]  # copy
    for i, n in moves:
        assert 0 < n <= state[i], "Illegal move"
        state[i] -= n
        if set(state) == {0}:
            return True  # you won!
        assert any(state), "You lost!"
        bot_move()

# Training problem 94
def f(probs: List[float]):
    assert len(probs) == 3 and abs(sum(probs) - 1) < 1e-6
    return max(probs[(i + 2) % 3] - probs[(i + 1) % 3] for i in range(3)) < 1e-6

# Training problem 95
def f(strategies: List[List[float]], A=[[1.0, -1.0], [-1.3, 0.8]], B=[[-0.9, 1.1], [0.7, -0.8]], eps=0.01):
    m, n = len(A), len(A[0])
    p, q = strategies
    assert len(B) == m and all(len(row) == n for row in A + B), "inputs are a bimatrix game"
    assert len(p) == m and len(q) == n, "solution is a pair of strategies"
    assert sum(p) == sum(q) == 1.0 and min(p + q) >= 0.0, "strategies must be non-negative and sum to 1"
    v = sum(A[i][j] * p[i] * q[j] for i in range(m) for j in range(n))
    w = sum(B[i][j] * p[i] * q[j] for i in range(m) for j in range(n))
    return (all(sum(A[i][j] * q[j] for j in range(n)) <= v + eps for i in range(m)) and
            all(sum(B[i][j] * p[i] for i in range(m)) <= w + eps for j in range(n)))

# Training problem 96
def f(edges: List[List[int]]):
    # first compute neighbors sets, N:
    N = {i: {j for j in range(99) if j != i and ([i, j] in edges or [j, i] in edges)} for i in range(99)}
    return all(len(N[i].intersection(N[j])) == (1 if j in N[i] else 2) for i in range(99) for j in range(i))

# Training problem 97
def f(tri: List[int], edges=[[0, 17], [0, 22], [17, 22], [17, 31], [22, 31], [31, 17]]):
    a, b, c = tri
    return [a, b] in edges and [b, c] in edges and [c, a] in edges and a != b != c != a

# Training problem 98
def f(path: List[int], weights=[{1: 20, 2: 1}, {2: 2, 3: 5}, {1: 10}], bound=11):
    return path[0] == 0 and path[-1] == 1 and sum(weights[a][b] for a, b in zip(path, path[1:])) <= bound

# Training problem 99
def f(path: List[int], edges=[[0, 11], [0, 7], [7, 5], [0, 22], [11, 22], [11, 33], [22, 33]], u=0, v=33, bound=3):
    assert path[0] == u and path[-1] == v and all([i, j] in edges for i, j in zip(path, path[1:]))
    return len(path) <= bound

# Training problem 100
def f(path: List[int], edges=[[0, 1], [0, 2], [1, 3], [1, 4], [2, 5], [3, 4], [5, 6], [6, 7], [1, 2]]):
    for i in range(len(path) - 1):
        assert [path[i], path[i + 1]] in edges
    assert path[0] == 0
    assert path[-1] == max(max(edge) for edge in edges)
    return True

# Training problem 101
def f(path: List[int], edges=[[0, 1], [0, 2], [1, 3], [1, 4], [2, 5], [3, 4], [5, 6], [6, 7], [1, 2]]):
    assert path[0] == 0 and path[-1] == max(max(e) for e in edges)
    assert all([[a, b] in edges for a, b in zip(path, path[1:])])
    return len(path) % 2 == 0

# Training problem 102
def f(p: List[int], edges=[[0, 1], [0, 2], [1, 3], [1, 4], [2, 5], [3, 4], [5, 6], [6, 7], [6, 1]]):
    return p[0] == 0 and p[-1] == 1 == len(p) % 2 and all([[a, b] in edges for a, b in zip(p, p[1:])])

# Training problem 103
def f(bi: List[int], g1=[[0, 1], [1, 2], [2, 3], [3, 4], [2, 5]], g2=[[0, 4], [1, 5], [4, 1], [1, 2], [2, 3]]):
    return len(bi) == len(set(bi)) and {(i, j) for i, j in g1} == {(bi[i], bi[j]) for i, j in g2}

# Training problem 104
def f(position: List[List[int]], transcript=[[[3, 3], [5, 5], [3, 7]], [[5, 3], [6, 4]]]):
    board = {(x, y): 0 for x in range(8) for y in range(8) if (x + y) % 2 == 0}  # empty board, 0 = empty
    for x, y, p in position:
        assert -2 <= p <= 2 and board[x, y] == 0  # -1, 1 is regular piece, -2, 2 is king
        board[x, y] = p

    def has_a_jump(x, y):
        p = board[x, y]  # piece to move
        deltas = [(dx, dy) for dx in [-1, 1] for dy in [-1, 1] if dy != -p]  # don't check backwards for non-kings
        return any(board.get((x + 2 * dx, y + 2 * dy)) == 0 and board[x + dx, y + dy] * p < 0 for dx, dy in deltas)

    sign = 1  # player 1 moves first
    for move in transcript:
        start, end = tuple(move[0]), tuple(move[-1])
        p = board[start]  # piece to move
        assert p * sign > 0, "Moving square must be non-empty and players must be alternate signs"
        assert all(board[x, y] == 0 for x, y in move if [x, y] != move[0]), "Moved to an occupied square"

        for (x1, y1), (x2, y2) in zip(move, move[1:]):
            assert abs(p) != 1 or (y2 - y1) * p > 0, "Non-kings can only move forward (in direction of sign)"
            if abs(x2 - x1) == 1:  # non-jump
                assert not any(has_a_jump(*a) for a in board if board[a] * p > 0), "Must make a jump if possible"
                break
            mid = ((x1 + x2) // 2, (y1 + y2) // 2)
            assert board[mid] * p < 0, "Can only jump over piece of opposite sign"
            board[mid] = 0
        board[start], board[end] = 0, p
        assert abs(x2 - x1) == 1 or not has_a_jump(*end)
        if abs(p) == 1 and any(y in {0, 7} for x, y in move[1:]):
            board[end] *= 2  # king me at the end of turn after any jumps are done!
        sign *= -1

    return True

# Training problem 105
def f(cut_position: int, ring="yRrsmOkLCHSDJywpVDEDsjgCwSUmtvHMefxxPFdmBIpM", lower=5):
    line = ring[cut_position:] + ring[:cut_position]
    matches = {c: 0 for c in line.lower()}
    for c in line:
        if c.islower():
            matches[c] -= (1 if matches[c] > 0 else len(line))
        else:
            matches[c.lower()] += 1
    return sum(i == 0 for i in matches.values()) >= lower

# Training problem 106
def f(nums: List[int], b=7, m=6):
    assert len(nums) == len(set(nums)) == m and min(nums) >= 0

    def gcd(i, j):
        r, s = max(i, j), min(i, j)
        while s >= 1:
            r, s = s, (r % s)
        return r

    for a in nums:
        nums = [(a + i + 1) ** 2 + (a + i + 1) + 1 for i in range(b)]
        assert all(any(i != j and gcd(i, j) > 1 for j in nums) for i in nums)

    return True

# Training problem 107
def f(indices: List[int], a0=123):
    assert a0 >= 0 and a0 % 3 == 0, "Hint: a_0 is a multiple of 3."
    s = [a0]
    for i in range(max(indices)):
        s.append(int(s[-1] ** 0.5) if int(s[-1] ** 0.5) ** 2 == s[-1] else s[-1] + 3)
    return len(indices) == len(set(indices)) == 1000 and min(indices) >= 0 and len({s[i] for i in indices}) == 1

# Training problem 108
def f(li: List[int], n=18):
    assert n % 3 == 0, "Hint: n is a multiple of 3"
    return len(li) == n and all(li[(i + 2) % n] == 1 + li[(i + 1) % n] * li[i] for i in range(n))

# Training problem 109
def f(inds: List[int], vecs=[169, 203, 409, 50, 37, 479, 370, 133, 53, 159, 161, 367, 474, 107, 82, 447, 385]):
    return all(sum((v >> i) & 1 for i in inds) % 2 == 1 for v in vecs)

# Training problem 110
def f(inds: List[int], vecs=[26, 5, 32, 3, 15, 18, 31, 13, 24, 25, 34, 5, 15, 24, 16, 13, 0, 27, 37]):
    return sum(sum((v >> i) & 1 for i in inds) % 2 for v in vecs) >= len(vecs) * 3 / 4

# Training problem 111
def f(nums: List[int]):
    a, b, c, n = nums
    return (a ** n + b ** n == c ** n) and min(a, b, c) > 0 and n > 2

# Training problem 112
def f(n: int, a=15482, b=23223, lower_bound=5):
    return a % n == 0 and b % n == 0 and n >= lower_bound

# Training problem 113
def f(n: int, nums=[77410, 23223, 54187], lower_bound=2):
    return all(i % n == 0 for i in nums) and n >= lower_bound

# Training problem 114
def f(n: int, a=15, b=27, upper_bound=150):
    return n % a == 0 and n % b == 0 and 0 < n <= upper_bound

# Training problem 115
def f(n: int, nums=[15, 27, 102], upper_bound=5000):
    return all(n % i == 0 for i in nums) and 0 < n <= upper_bound

# Training problem 116
def f(nums: List[int], n=12345):
    return len(nums) <= 4 and sum(i ** 2 for i in nums) == n

# Training problem 117
def f(li: List[int], k=5):
    def prod(nums):
        ans = 1
        for i in nums:
            ans *= i
        return ans

    return min(li) > 1 and len(li) == k and all((1 + prod(li[:i] + li[i + 1:])) % li[i] == 0 for i in range(k))

# Training problem 118
def f(n: int):
    m = n
    while n > 4:
        n = 3 * n + 1 if n % 2 else n // 2
        if n == m:
            return True

# Training problem 119
def f(start: int):
    n = start  # could be positive or negative ...
    while abs(n) > 1000:
        n = 3 * n + 1 if n % 2 else n // 2
        if n == start:
            return True

# Training problem 120
def f(n: int, t=197, upper=20):
    m = n
    for i in range(t):
        if n <= 1:
            return False
        n = 3 * n + 1 if n % 2 else n // 2
    return n == 1 and m <= 2 ** upper

# Training problem 121
def f(n: int):
    return pow(2, n, n) == 3

# Training problem 122
def f(n: int, year_len=365):
    import random
    random.seed(0)
    K = 1000  # number of samples
    prob = sum(len({random.randrange(year_len) for i in range(n)}) < n for j in range(K)) / K
    return (prob - 0.5) ** 2 <= year_len

# Training problem 123
def f(counts: List[int], target_prob=0.5):
    m, n = counts  # m = num 1's, n = num -1's
    probs = [1.0] + [0.0] * n  # probs[n] is probability for current m, starting with m = 1
    for i in range(2, m + 1):  # compute probs using dynamic programming for m = i
        old_probs = probs
        probs = [1.0] + [0.0] * n
        for j in range(1, min(n + 1, i)):
            probs[j] = (
                    j / (i + j) * probs[j - 1]  # last element is a -1 so use probs
                    +
                    i / (i + j) * old_probs[j]  # last element is a 1 so use old\_probs, m = i - 1
            )
    return abs(probs[n] - target_prob) < 1e-6

# Training problem 124
def f(s: str):
    return s + 'world' == 'Hello world'

# Training problem 125
def f(st: str, a="world", b="Hello world"):
    return st + a == b

# Training problem 126
def f(s: str, n=1000):
    return len(s) == n

# Training problem 127
def f(inds: List[int], s="hello world", target="do"):
    i, j, k = inds
    return s[i:j:k] == target

# Training problem 128
def f(s: str, big_str="foobar", index=2):
    return big_str.index(s) == index

# Training problem 129
def f(big_str: str, sub_str="foobar", index=2):
    return big_str.index(sub_str) == index

# Training problem 130
def f(s: str, a="hello", b="yellow", length=4):
    return len(s) == length and s in a and s in b

# Training problem 131
def f(substrings: List[str], s="hello", count=15):
    return len(substrings) == len(set(substrings)) >= count and all(sub in s for sub in substrings)

# Training problem 132
def f(string: str, substring="a", count=10, length=100):
    return string.count(substring) == count and len(string) == length

# Training problem 133
def f(x: str, parts=['I!!', '!love', 'dumplings', '!', ''], string="I!!!!!love!!dumplings!!!!!"):
    return x.join(parts) == string

# Training problem 134
def f(parts: List[str], sep="!!", string="I!!!!!love!!dumplings!!!!!"):
    return sep.join(parts) == string and all(sep not in p for p in parts)

# Training problem 135
def f(li: List[int], dups=42155):
    return len(set(li)) == len(li) - dups

# Training problem 136
def f(li: List[int], target=[17, 9, -1, 17, 9, -1], n=2):
    return li * n == target

# Training problem 137
def f(i: int, li=[17, 31, 91, 18, 42, 1, 9], target=18):
    return li[i] == target

# Training problem 138
def f(i: int, li=[17, 31, 91, 18, 42, 1, 9], target=91):
    return li[i] == target and i < 0

# Training problem 139
def f(inds: List[int], li=[42, 18, 21, 103, -2, 11], target=[-2, 21, 42]):
    i, j, k = inds
    return li[i:j:k] == target

# Training problem 140
def f(s: str, a=['cat', 'dot', 'bird'], b=['tree', 'fly', 'dot']):
    return s in a and s in b

# Training problem 141
def f(x: int, a=93252338):
    return -x == a

# Training problem 142
def f(x: int, a=1073258, b=72352549):
    return a + x == b

# Training problem 143
def f(x: int, a=-382, b=14546310):
    return x - a == b

# Training problem 144
def f(x: int, a=8665464, b=-93206):
    return a - x == b

# Training problem 145
def f(n: int, a=14302, b=5):
    return b * n + (a % b) == a

# Training problem 146
def f(n: int, a=3, b=23463462):
    return b // n == a

# Training problem 147
def f(n: int, a=345346363, b=10):
    return n // b == a

# Training problem 148
def f(x: int, a=10201202001):
    return x ** 2 == a

# Training problem 149
def f(x: float, a=1020):
    return abs(x ** 2 - a) < 10 ** -3

# Training problem 150
def f(x: float, a=1020):
    return abs(x ** 2 - a) < 10 ** -3 and x < 0

# Training problem 151
def f(s: str):
    return "Hello " + s == "Hello world"

# Training problem 152
def f(s: str):
    return "Hello " + s[::-1] == "Hello world"

# Training problem 153
def f(x: List[int]):
    return len(x) == 2 and sum(x) == 3

# Training problem 154
def f(s: List[str]):
    return len(set(s)) == 1000 and all((x.count("a") > x.count("b")) and ('b' in x) for x in s)

# Training problem 155
def f(n: int):
    return str(n * n).startswith("123456789")

\end{pylittledisplay}

